Encoding of Predicate Subtyping with Proof Irrelevance in the $\lambda$$\Pi$-Calculus Modulo Theory

The $\lambda$$\Pi$-calculus modulo theory is a logical framework in which various logics and type systems can be encoded, thus helping the cross-verification and interoperability of proof systems based on those logics and type systems. In this paper, we show how to encode predicate subtyping and proof irrelevance, two important features of the PVS proof assistant. We prove that this encoding is correct and that encoded proofs can be mechanically checked by Dedukti, a type checker for the $\lambda$$\Pi$-calculus modulo theory using rewriting.

==> conservativity.tex <==
\subsection{Conservativity}
\begin{definition}[Inverse translation]
  The \emph{inverse term translation} \(\trZobji{M}\) is partially defined by
  induction on \(M\) in \cref{fig:inverse-term-translation}.
\end{definition}
\begin{figure}
    \begin{gather*}
      \trZobji{x} = x\\
      \trZobji{\teZabst{x}[T]{M}} = \teZabst{x}[\trZtypi{T}]{\trZobji{M}}
\\
      \trZobji{M~N} = \trZobji{M}~\trZobji{N}
\\
      \trZobji{\ecZbool} = \teZProp
\\
      \trZobji{\ecZfa T\,(\teZabst{x}[\square]{U})} =
      \teZprod{x}{\trZobji{T}}{\trZobji{U}}
\\
      \trZobji{P \ecZimpd (\teZabst{x}[\square]{Q})} =
      \teZprod{x}{\trZobji{P}}{\trZobji{Q}}
\\
      \trZobji{T \ecZarrd (\teZabst{x}[\square]{Q})} =
      \teZprod{x}{\trZobji{T}}{\trZobji{Q}}
\\
      \trZobji{\ecZpsub T\,P} =
      \teZpsub{\trZobji{T}}{\trZobji{P}}
\\
      \trZobji{\ecZpair T\,P\,M\,N} =
      \teZpair{\trZobji{T}}{\trZobji{P}}{\trZobji{M}}{\trZobji{N}}
\\
      \trZobji{\ecZfst T\,P\,M} =
      \teZprol{\trZobji{T}}{\trZobji{P}}{\trZobji{M}}
\\
      \trZobji{\ecZsnd T\,P\,M} =
      \teZpror{\trZobji{T}}{\trZobji{P}}{\trZobji{M}}
    \end{gather*}
  \caption{Inverse term translation.}\label{fig:inverse-term-translation}
\end{figure}

\begin{definition}[Inverse type translation]
  The \emph{inverse type translation} \(\trZtypi{T}\) is partially defined by
  induction on \(T\) in \cref{fig:inverse-type-translation}.
\end{definition}
\begin{figure}
  \begin{minipage}{0.5\textwidth}
    \begin{gather*}
      \trZtypi{\ecZSet} = \teZType\\
      \trZtypi{\ecZBool} = \teZProp
    \end{gather*}
  \end{minipage}
  \begin{minipage}{0.5\textwidth}
    \begin{gather*}
      \trZtypi{\ecZEl M} = \trZobji{M}\\
      \trZtypi{\ecZPrf P} = \trZobji{P}\\
      \trZtypi{\teZprod{x}{T}{U}} = \teZprod{x}{\trZtypi{T}}{\trZtypi{U}}
    \end{gather*}
  \end{minipage}
  \caption{Inverse type translation.}\label{fig:inverse-type-translation}
\end{figure}

\begin{lemma}[Inverse]
  For all \(\Gamma, M, T\), if \(\Gamma \jgZpvs M: T\),
  then \(\trZobji{\trZobj{M}_{\Gamma}} \rlZcov_{\beta} M\).
\end{lemma}
\begin{proof}
  \todo[inline]{Update proof regarding new translation (restricted to applied
    terms)}
  By structural induction on \(M\), the cases for \(\ecZpsub\) and \(\ecZpair\)
  are detailed.
  \begin{description}
    \item[Case \(M = \teZpsub{T}{U}\),]
      then we have \(\trZobj{M}_{\Gamma} =
      \ecZpsub \trZobj{T}_{\Gamma}~(\teZabst{x}[\trZtyp{T}]{\trZobj{U}_{\Gamma, x: T}})\)
      and
      \begin{align*}
        \trZobji{\trZobj{M}_{\Gamma}}
        &= \left(
          \teZabstp{\tau}[\teZType]
          \teZabstp{\upsilon}[\tau \teZarr \teZProp]\teZpsub{x'}{\tau}{\upsilon~x'}\right)
          \trZobji{\trZobj{T}_{\Gamma}}~\left(\teZabstp{x}[\trZtypi{\trZtyp{T}_{\Gamma}}]
          \trZobji{\trZobj{U}_{\Gamma, x:T}}\right)
        \\
        &\rlZcov_{\beta} \teZpsub{x'}{\trZobji{\trZobj{T}_{\Gamma}}}{%
          \left(\teZabstp{x}[\trZtypi{\trZtyp{T}_{\Gamma}}]
          \trZobji{\trZobj{U}_{\Gamma, x:T}}\right)~x'
          }
        \\
        &= \teZpsub{x'}{T}{\left(\teZabstp{x}[T]U\right)~x'} \text{ by induction hypothesis}
        \\
        &\rlZcov_{\beta} \teZpsub{T}{U}
      \end{align*}
    \item[Case \(M = \teZpair{}{T}{M}{N}\),]
      because \(M\) is well typed, we have \(T\) of the form
      \(T = \teZpsub{T_{0}}{U_{0}}\), hence
      \(\trZobj{M}_{\Gamma} = \ecZpair \trZobj{T_{0}}_{\Gamma}~\left(\teZabstp{x}[\trZtyp{T_{0}}]
      \trZobj{U_{0}}_{\Gamma, x: T_{0}}\right)\), hence
      \begin{align*}
        \trZobji{\trZobj{M}_{\Gamma}}
        &=
          \begin{multlined}
            \left(
              \teZabstp{\tau}[\teZType]
              \teZabstp{\upsilon}[\tau \teZarr \teZProp]
              \teZabstp{\mu}[\tau]\teZabstp{\nu}[\upsilon~\mu]
              \teZpair{\tau}{\teZabst{x}{\upsilon\,x}}{\mu}{\nu}
            \right)\\
            \trZobji{\trZobj{T}_{\Gamma}}~
            \left(\teZabstp{x}[\trZtypi{\trZtyp{T}_{\Gamma}}]
              \trZobji{\trZobj{U}_{\Gamma, x:T}}\right)~
            \trZobji{\trZobj{M}_{\Gamma}}~
            \trZobji{\trZobj{N}_{\Gamma}}
          \end{multlined}
        \\
        &=
          \begin{multlined}
            \left(
              \teZabstp{\tau}[\teZType]
              \teZabstp{\upsilon}[\tau \teZarr \teZProp]
              \teZabstp{\mu}[\tau]\teZabstp{\nu}[\upsilon~\mu]
              \teZpair{\tau}{\teZabst{x}{\upsilon\, x}}{\mu}{\nu}
            \right)\\
            T~\left(\teZabstp{x}[\trZtypi{\trZtyp{T}_{\Gamma}}]
              U\right)~M~N
          \end{multlined}\text{ by induction hypothesis}
        \\
        &= \teZpair{T}{%
          \left(\teZabstp{x}[\trZtypi{\trZobj{T}_{\Gamma, x:T}}] U\right)~x}{M}{N}
        \\
        &\rlZcov_{\beta} \teZpair{T}{U}{M}{N}
          \qedhere
      \end{align*}
  \end{description}
\end{proof}

\begin{corollary}
  For all \(\Gamma, T\), if \(\Gamma \jgZpvs T: s\),
  then \(\trZtypi{\trZobj{T}_{\Gamma}} \pcZdeq T\).
\end{corollary}

To prove conservativity of equivalence, we need a lemma similar to
\cref{prop:pcert-eq-confluence}.

\begin{lemma}
  Let \(M\) and \(N\) be two well typed terms of \lpme\todo{of the encoding}.
  If \(M \lpZdeq N\), then \(\trZobji{M} \pcZdeq \trZobji{N}\).
\end{lemma}
\begin{proof}

\end{proof}

